Robotic Computing on FPGAs: Current Progress, Research Challenges, and Opportunities

Robotic computing has reached a tipping point, with a myriad of robots (e.g., drones, self-driving cars, logistic robots) being widely applied in diverse scenarios. The continuous proliferation of robotics, however, critically depends on efficient computing substrates, driven by real-time requirements, robotic size-weight-and-power constraints, cybersecurity considerations, and dynamically changing scenarios. Within all platforms, FPGA is able to deliver both software and hardware solutions with low power, high performance, reconfigurability, reliability, and adaptivity characteristics, serving as the promising computing substrate for robotic applications. This paper highlights the current progress, design techniques, challenges, and open research challenges in the domain of robotic computing on FPGAs.

==> 6acknowledgemnt.tex <==
\section*{Acknowledgements}
This work was supported in part by C-BRIC, one of six centers in JUMP, a Semiconductor Research Corporation (SRC) program sponsored by DARPA.

==> tabs/library.tex <==
\begin{table}[t!]
\centering
\caption{[Placeholder] Algorithm modular and libraries.}
\vspace{-3pt}
\renewcommand*{\arraystretch}{1.1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Abstraction}\\ \textbf{Layer} \end{tabular} & \textbf{Platform}                                                                 & \begin{tabular}[c]{@{}c@{}}\textbf{Perf.}\\ \textbf{(cycles/sec)} \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Exec.}\\ \textbf{Time (1 run)} \end{tabular}  & \begin{tabular}[c]{@{}c@{}}\textbf{Exec.}\\ \textbf{Time (1000 runs)} \end{tabular} \\ \hline

RTL                  & \begin{tabular}[c]{@{}c@{}}IVM Alpha-like processor\\ RTL simulation~\cite{maniatakos2010instruction} \end{tabular} & 6$\times$$10^2$     & 4.2$\times$$10^{5}$ hours               & 1.74$\times$$10^{7}$days                 \\ \hline 

Micro-architecture         & gem5 simulator~\cite{binkert2011gem5}                                                                    & 3$\times$$10^6$     & 83.3 hours                 & 3472 days                    \\ \hline
\begin{tabular}[c]{@{}c@{}}FPGA Emulation \end{tabular}   & \begin{tabular}[c]{@{}c@{}}OpenSPARC T1\\ FPGA emulation~\cite{pellegrini2012crashtest} \end{tabular}                                                     & 1$\times$$10^7$     & 25 hours                   & 1040 days                     \\ \hline

Architecture               & TSIM SPARC simulator~\cite{danvek2013leon3}                                                              & 6$\times$$10^7$     & 4.17 hours                 & 173.6 days                    \\ \hline



Software (Ours)            & x86 processor~\cite{yim2010measurement}                                                                     & 3$\times$$10^9$     & 5 mins                     & 3.48 days                    \\ \hline

\end{tabular}
}
% \caption{Compute time overhead of anomaly detection and recovery scheme for each stage. }
\label{tab:FI_compare}
\vspace{-5pt}
\end{table}

